Specifying, Monitoring, and Executing Workflows in Linked Data Environments

We present an ontology for representing workflows over components with Read-Write Linked Data interfaces and give an operational semantics to the ontology via a rule language. Workflow languages have been successfully applied for modelling behaviour in enterprise information systems, in which the data is often managed in a relational database. Linked Data interfaces have been widely deployed on the web to support data integration in very diverse domains, increasingly also in scenarios involving the Internet of Things, in which application behaviour is often specified using imperative programming languages. With our work we aim to combine workflow languages, which allow for the high-level specification of application behaviour by non-expert users, with Linked Data, which allows for decentralised data publication and integrated data access. We show that our ontology is expressive enough to cover the basic workflow patterns and demonstrate the applicability of our approach with a prototype system that observes pilots carrying out tasks in a mixed-reality aircraft cockpit. On a synthetic benchmark from the building automation domain, the runtime scales linearly with the size of the number of Internet of Things devices.

==> sections/ivision.tex <==

We used the approach presented in this paper in the \ivision project\footnote{\url{http://www.ivision-project.eu/}}. 
The \ivision project was about the Human Factors (HF)-based evaluation of aircraft cockpits regarding pilot workflows.
To perform the evaluation early in the design process, virtual models of aircraft cockpits are used.

We used the ontology to formalise hierarchical task analysis (HTA) models.
HF-based evaluation of workflows is traditionally done using the method HTA from occupational psychology~\cite{HTAoriginal1967}.
HTA is a pen-and-paper-based method to hierarchically decompose workflows.
The resulting workflow model is tree-shaped, but the specification is not formally grounded.
To work with the formal methods from workflow management, we formalised the traditionally textual description of control flow (so-called plans) in HTA.
For the formalisation, we restricted the control flow to the most common plans from HTA, and provided an analogy for those plans from workflow management:
the basic workflow patterns plus the unordered sequence.

We used the ontology and the operational semantics in the \ivision system to observe pilot workflows in Virtual Reality.
The \ivision system to analyse virtual aircraft cockpits using HTA is composed of a HF-enabled Virtual Reality rendering engine displaying a virtual aircraft cockpit, a flight simulator, and our workflow observation.
A pilot then gets immersed to the aircraft cockpit using Virtual Reality glasses.
The pilot can interact with the virtual cockpit using finger tracking, which translates his movements to interactions with the virtual aircraft, whose dynamics are implemented in the flight simulator.
We built a Linked Data interface to the flight simulator and the renderer to expose data about the current state of affairs in the cockpit such that the data is available for querying, \eg in SPARQL ASK queries in the postconditions.
Our workflow observation subsystem has been set-up like described in this paper.
All system components were connected using Ethernet.
Both the Linked Data Platform implementation and the Linked Data-Fu engine are installed on an off-the-shelf quad-core laptop running Windows 10 64-bit and Java 8.
The un-optimised implementation ran at 2\,Hz, sufficient for the use-case.
Previously, we built a similar, but optimised set-up, which supported update rates up to 30\,Hz~\cite{DBLP:conf/ismar/KeppmannKSSH14}, the update rate of a Microsoft Kinect sensor.


In \ivision, our observation approach automatises the traditional manual HF data collection using stopwatches.
On top of this data collection, we facilitated run-time analysis of cockpits:
Leveraging the stack of semantic technologies, we can answer structured queries given in SPARQL posed against the whole system at run-time such as \enquote{which are all the buttons that are to be pressed in the upcoming steps of the currently running workflow instance?}.


==> sections/scenario.tex <==
Similar to the IoT domain, fragmentation of technologies is also an issue in the area of building automation:
NIST identified interoperability as major challenge for the building industry~\cite{gcr2004cost}.
\citeauthor*{DBLP:conf/sensys/BalajiBFGGHJKPA16} aim to raise interoperability in Building Management Systems (BMS) using Semantic Technologies:
Using the Brick ontology~\cite{DBLP:conf/sensys/BalajiBFGGHJKPA16}, people can model buildings and corresponding BMSs.
Read-Write Linked Data interfaces to a building's BMSs allow for executing automation tasks for the building.
Such tasks can include:
\begin{inparaenum}[(1)]
\item \label{enum:tasks:timecontrol}Control schemes based on time, sensor data and web data,
\item Automated supervision of cleaning personnel,
\item Presence simulation,
\item Evacuation support.
\end{inparaenum}
Those tasks go beyond simple rule-based automation tasks as typically found in home automation (\eg Eclipse SmartHome\footnote{\url{https://www.eclipse.org/smarthome/}}) and on the web (\eg IFTTT\footnote{\url{https://ifttt.com/}}), as the tasks require a notion of task instance state.
We therefore model the tasks as workflow and run them as workflow instances, which access the building management systems in an integrated fashion using the Read-Write Linked Data interfaces.

As building, we use a description of building 3 at IBM Research Dublin in Ireland.
\citeauthor*{DBLP:conf/sensys/BalajiBFGGHJKPA16} provide a static description of the building using the Brick ontology\footnote{\label{foot:IBM_B3}\url{https://github.com/BuildSysUniformMetadata/GroundTruth/blob/2e48662/building_instances/IBM_B3.ttl}}.
The description covers the building's parts (\eg rooms) and the parts of the building's systems (\eg lights and switches).
We serve the description on a Linked Data interface.
To add state information to the systems, we add writeable properties from the SSN ontology\footnote{\url{https://www.w3.org/TR/vocab-ssn/}} to the Linked Data interface.

